The decomposition of optimal transportation problems with convex cost

Given a positive l.s.c. convex function $\mathtt c : \mathbb R^d \to \mathbb R^d$ and an optimal transference plane $\underline{\pi}$ for the transportation problem \begin{equation*} \int \mathtt c(x'-x) \pi(dxdx'), \end{equation*} we show how the results of \cite{biadan} on the existence of a \emph{Sudakov decomposition} for norm cost $\mathtt c= |\cdot|$ can be extended to this case. More precisely, we prove that there exists a partition of $\mathbb R^d$ into a family of disjoint sets $\{S^h_\mathfrak a\}_{h,\mathfrak a}$ together with the projection $\{O^h_\mathfrak a\}_{h,\mathfrak a}$ on $\mathbb R^d$ of proper extremal faces of $\mathrm{epi}\, \mathtt c$, $h = 0,\dots,d$ and $\mathfrak a \in \mathfrak A^h \subset \mathbb R^{d-h}$, such that - $S^h_\mathfrak a$ is relatively open in its affine span, and has affine dimension $h$; \item $O^h_\mathfrak a$ has affine dimension $h$ and is parallel to $S^h_\mathfrak a$; - $\mathcal L^d(\mathbb R^d \setminus \cup_{h,\mathfrak a} S^h_\mathfrak a) = 0$, and the disintegration of $\mathcal L^d$, $\mathcal L^d = \sum_h \int \xi^h_\mathfrak a \eta^h(d\mathfrak a)$, w.r.t. $S^h_\mathfrak a$ has conditional probabilities $\xi^h_\mathfrak a \ll \mathcal H^h \llcorner_{S^h_\mathfrak a}$; - the sets $S^h_\mathfrak a$ are essentially cyclically connected and cannot be further decomposed. \end{list} The last point is used to prove the existence of an optimal transport map. The main idea is to recast the problem in $(t,x) \in [0,\infty] \times \mathbb R^d$ with an $1$-homogeneous norm $\bar{\mathtt c}(t,x) := t \mathtt c(- \frac{x}{t})$ and to extend the regularity estimates of \cite{biadan} to this case.

==> structure3.tex <==

\section{Sketch of proof and structure of the paper}
\label{S_struct_sudakov_paper}


\subsection{Sketch of the proof}
\label{Ss_sketch}


In the first part of this section we will give an overview proof of the construction of the subpartition of a given locally affine partition in the spirit of the construction made by Bianchini and Daneri in \cite{BiaDan}. The idea is to avoid the details and to underline the main ideas, in order to help (or avoid) the reading of the next sections. For the notation we refer to Section \ref{S_setting}.


\subsubsection{Locally affine partitions}
\label{Sss_loca_afi}

Contrary to \cite{BiaDan} we have to deal with a partition of $[0,+\infty)\times\R^d$. Let $\{Z^k_\mathfrak a\}_{k,\mathfrak a}$ be a partition of $[0,+\infty)\times\R^d$ into sets which are locally affine: this means that they are relatively open in the affine space $\aff\,Z^k_\mathfrak a$ generated by themselves. The index $k$ is referred to the dimension of the set, while $\mathfrak a$ is an index.

To each of these sets it is attached a convex cone $C^k_\mathfrak a$, parallel to $\aff\,Z^k_\mathfrak a$, which is not degenerate: it is strictly contained in a half $k$-dimensional plane, and it is really $k$-dimensional, meaning that its span is $k$-dimension. Moreover, we require that $C^k_\mathfrak a\cap(\{1\}\times\R^d)$ is a convex $(k-1)-$dimensional convex. This request will be clear later.

{\color{red} perche'?}
Since the dependence of $(k,\mathfrak a) \mapsto (Z^k_\mathfrak,C^k_\mathfrak a)$ is $\sigma$-continuous (i.e. its graph is a countable union of compact sets), it is a standard decomposition arguments to divide the partition into countably many partitions with the following properties:
\begin{enumerate}
	\item \label{Point_k_dime}  	the dimension $k$ is constant,
	\item \label{Point_closeredf} 	the spaces $\aff\,Z^k_\mathfrak a$ have direction close to a given $k$-dimensional reference plane,
	\item \label{Point_unicon} 		 the cones $C^k_\mathfrak a$, when projected on this reference plan, strictly contains and are contained in two given non degenerate cones,
	\item \label{Point_contaQ} 		the projection of $Z^k_\mathfrak a$ contains a given $k$-dimensional cube $Q$.
\end{enumerate}
The properties \eqref{Point_closeredf}, \eqref{Point_contaQ} imply that we can take as quotient space the $(d+1-k)$-dimensional subspace orthogonal to a point in $Q$. This will be the default choice for $\mathfrak a$.

Two measures are associated with the directed locally affine partition: a transference plan $\bar\pi$, whose first marginal $\bar\mu := (\mathtt p_1)_\sharp \bar\pi$ is concentrated on $\mathbf Z_1 := \cup Z^k_\mathfrak a \cap (\{1\}\times\R^d)$ and such that it has finite cost w.r.t.
\[
	\mathtt c_{\mathbf Z}(z,z') :=
		\begin{cases}
			0 & z \in Z^k_\mathfrak a, z' - z \in C^k_\mathfrak a, \crcr
			\infty & \text{otherwise},
		\end{cases}
\]
and the Lebesgue measure on $\mathbf Z_1$. The starting assumption on $\mathcal H^d \llcorner_{\mathbf Z_1}$ is the regularity of the disintegration
\[
	\mathcal H^d \llcorner_{\mathbf Z_1} = \sum_k \int \upsilon^k_\mathfrak a \eta^k(d\mathfrak a)
\]
as follows: $\upsilon^k_\mathfrak a \sim \mathcal H^k \llcorner_{Z^k_\mathfrak a}$ and $\eta^k \ll \mathcal H^{d+1-k}$.


\subsubsection{Mapping a partition to a fibration}
\label{Sss_map_part_fibra}


By projecting $(Z^k_\mathfrak a,C^k_\mathfrak a)$ on the product space $\R^{d+1-k} \times \R^k$, we obtain a structure of the following form: for all $\mathfrak a \in \R^{d+1-k}$ there are sets $\tilde Z^k_\mathfrak a$, $\tilde C^k_\mathfrak a$ (the projection of $Z^k_\mathfrak a$, $C^k_\mathfrak a$) such that $Q \subset \tilde Z^k_\mathfrak a$ and $\tilde C^k_\mathfrak a = \epi \mathtt{co}_\mathfrak a$ for some $1$-homogeneous convex uniformly Lipschitz functions $\mathtt{co}_\mathfrak a: \R^{k-1} \mapsto \R$: the last property follows from Point \eqref{Point_unicon} above. 

We will call the above structure a fibration. Notice that since the projection map from $\aff\,Z^k_\mathfrak a$ to the reference $k$-dimensional plane is invertible with uniform Lipschitz bounds, the assumptions on the disintegration of $\mathcal H^d \llcorner_{\mathbf Z_1}$ are equivalent to Fubini's theorem on a fibration. %Instead, since the projection is invertible only on $\tilde Z^k_\mathfrak a$, to pass transference plans we need to specify the decomposition
% \[
% \nu = \sum_k \int \nu^k_\mathfrak a \xi^k(d\mathfrak a)
% \]
% of second marginal $\nu$ of $\pi$ as follows:
% \[
% \pi = \sum_k \int \pi^k_\mathfrak a \xi^k(d\mathfrak a), \quad \nu ^k_\mathfrak a := (\mathtt p_2)_\sharp \pi^k_\mathfrak a.
% \]
Moreover we need only to study the refinement of the fibration $\tilde Z^k_\mathfrak a,\tilde C^k_\mathfrak a$, and to map it back to the original directed locally affine partition.

We notice here that the image $\bar \nu$ of the second marginal $\bar \nu := (\mathtt p_2)_\sharp \bar \pi$ is defined through the decomposition
\[
\bar \nu = \sum_k \int \bar \nu^k_\mathfrak a \xi^k(d\mathfrak a),
\]
where
\[
\bar \pi = \sum_k \int \bar \pi^k_\mathfrak a \xi^k(d\mathfrak a), \quad \bar \nu ^k_\mathfrak a := (\mathtt p_2)_\sharp \bar \pi^k_\mathfrak a.
\]


\subsubsection{Construction of a linear preorder}
\label{Sss_line_preord_fiber}


The construction of the refinement is now done simultaneously on every fiber $\mathfrak a + \R^k$. For simplicity we will explain how to do it on a single fiber, since the general case is an application of basic descriptive set theory techniques. We will write $\tilde Z^k$, $\tilde C^k$, $\tilde \mu^k$, $\tilde \nu^k$, $\tilde \pi^k$, i.e. we assume $\mathfrak a$ fixed and we will omit it. Moreover, we will omit the symbol used for the reference structure ($\tilde \cdot$).

The first step is the construction of a linear preorder $\preccurlyeq$ with the following properties:
\begin{enumerate}
	\item it has Borel graph,
	\item it contains the set $\{(w,w') \in \R^k \times \R^k : w' - w \in C^k\}$,
	\item the equivalence classes with positive $\mu$-measure are cyclically connected up to a $ \mu^k$-negligible set.
\end{enumerate}
The last point means the following: for all transference plan $\pi^k \in \Pi^f_{ C^k}( \mu^k, \nu^k)$, all points in the classes of positive $\mu^k$-measure are cyclically connected, i.e. there exists a closed cycle of finite $ C^k$-cost passing through any couple of points $w$, $w'$, up to a $ \mu$-negligible set.

The first step is to define the set of points $H_{\bar w}$ which can be reached from a given point $\bar w$ by means of axial path of finite cost. It can be shown that, due to the non degeneracy of $ C^k$, this set is given by
\[
	\big\{ (x,y) \in \R^{k-1} \times \R, y \leq \mathtt h_{\bar w}(x) \big\}
\]
for some Lipschitz function $\mathtt h_{\bar w} : \R^{k-1} \mapsto \R$. Moreover, since we can always assume that $\Id \subset \Gamma$, we have $\bar w \in H_{\bar w}$.

For any countable choice of $\bar w_\beta$, $\Gamma_\beta$, $\beta < \alpha$ with $\alpha < \Omega$, we can thus construct the function
\[
\R^k \ni w \mapsto \theta(w) := \Big( \chi_{H_{\bar w_1}}(w), \chi_{H_{\bar w_2}}(w), \dots \Big) \in \{0,1\}^\alpha,
\]
and the preorder $\preccurlyeq$ is the inverse image of the lexicographic preorder on $\{0,1\}^\alpha$. It is fairly easy to see that the family of equivalence relations $\preccurlyeq \cap \preccurlyeq^{-1}$ is closed under countable intersection, by concatenating countably many preorders.


\subsubsection{Minimal equivalence relation and cyclical connected equivalence classes}
\label{Sss_min_conn_clas}


By Theorem \ref{T_minimal_equival} there exists a minimal equivalence relation $\bar E$, corresponding to a function $\bar \theta$: Corollary \ref{C_constant_for_minimal_equivalence} implies that $H_w$ essentially contains or it is essentially disjoint by all equivalence classes of positive $ \mu^k$-measure.

In particular, if $ \mu^k \ll \mathcal H^{k-1}$, then the Lebesgue points of the set $\{d \mu^k \slash d\mathcal H^{k-1} > 0\} \cap \{\bar \theta = \mathrm{const}\}$ are cyclically connected for all $\bar \Gamma$. Indeed, if $w$, $w'$ are Lebesgue points, then $w' \in H_w$, otherwise by the Lipschitz properties of $\mathtt h_w$ the set $( w' + C^k) \cap H_w = \emptyset$, while it has positive Lebesgue measure in $\{\bar \theta = \mathrm{const}\}$. We thus have a contradiction.

We notice here that, due to the Lipschitz regularity of $\mathtt h_{\bar w}$, it is possible to prove that the level sets with positive Lebesgue measure are bounded by two Lipschitz graphs, a regularity property finer that the relative opening.


\subsubsection{Decomposition of the level sets of $\bar \theta$}
\label{Sss_deco_leve_bar_thet}


Next, we decompose the level sets of $\bar \theta$ which are $\mathcal H^d$-negligible: in this decomposition we will obtain a residual set, which will be shown to be $\mathcal H^{k-1}$-negligible.

The good set $R$ is made of points $w$ such that:
\begin{enumerate}
\item \label{Point_future_good} the intersection
\[
\big\{ w': \bar \theta(w') = \bar \theta(w) \big\} \cap \big( w +  CK k\big)
\]
is the restriction to $\{ w': \bar \theta(w') = \bar \theta(w) \}$ of an $\ell$-dimensional subcone $C'^\ell_\mathfrak c$ of $ C^k$, $\mathfrak c$ being a generic index,
\item \label{Point_past_good} the intersection
\[
\big\{ w': \bar \theta(w') = \bar \theta(w) \big\} \cap \big( w - C^k \big)
\]
is the restriction to $\{ w': \bar \theta(w') = \bar \theta(w) \}$ of $- C'^\ell_\mathfrak c$,
\item \label{Point_before_ok} there is a point $w^-$ in
\[
\big\{ w': \bar \theta(w') = \bar \theta(w) \big\} \cap \big( w - \interr  C^k \big)
\]
satisfying the above two conditions,
\item \label{Point_after_ok} there is a point $w^+$ in
\[
\big\{ w': \bar \theta(w') = \bar \theta(w) \big\} \cap \big( w + \interr  C^k \big)
\] 
satisfying the above 2 conditions.
\end{enumerate}

By the convexity properties of $C^k$, it is fairly easy to see that
\[
w \in \interr Q(w^-,w^+) := \big( w^- + C^k \big) \cap \big( w^+ -  C^k \big) \subset \big\{ w': \bar \theta(w') = \bar \theta(w) \big\},
\]
which means that the set $Z'^\ell_\mathfrak c$ made of all points satisfying the above points and lying in the same affine space $\aff\,(w + C'^\ell_\mathfrak c)$ is relatively open.

It can be shown that the residual set is made of points which are relative boundaries of the sets $R^+$ or $R^-$, where $w \in \R^k$ if only Conditions \eqref{Point_future_good}, \eqref{Point_before_ok} of page \pageref{Point_future_good}, and the other two conditions for $w \in R^-$: in the first case we will call them the set of initial points, and in the other end points.

A countable partition of $R$ as in Point \eqref{Point_k_dime}, \eqref{Point_closeredf}, \eqref{Point_unicon}, \eqref{Point_contaQ} of page \pageref{Point_k_dime} implies that it is enough to study a family of elements $ Z'^\ell_\mathfrak c$, with $\ell$-fixed and projecting on a given $\ell$-dimensional cube.

{\color{blue}
\subsubsection{Negligibility of the residual set and absolute continuity of the disintegration}
\label{Sss_negli_absol}


By slicing the sets $Z'^\ell_\mathfrak c$ along a $k-\ell+1$-plane whose intersection with $\aff\,Z'^\ell_\mathfrak c$ is a $1$-dimensional direction contained in $\interr  C'^\ell_\mathfrak c$, we reduce to the case were $\ell = 1$. The results will be proved in this case, and the extension is only a matter of taking $\ell$-independent directions and repeating the estimates.

Take two $(d-1)$-dimensional planes $F$, $F'$ orthogonal to the reference segment $Q$ and passing on the initial and final point of the segment $Q$: by the definition of $Q$, it follows that $F$, $F'$ are transversal to the segments $ Z'^1_\mathfrak c$ and the direction of the cones $ C'^1_\mathfrak c$ points from $F$ to $F'$. The fact that $\ell = 1$ implies that, for every point $x \in \tilde Z'^1_\mathfrak c ca\ F$, the intersection of the level set of $\{\bar \theta = \bar \theta(x)\}$ with $x +  C'^1_\mathfrak c$ is the single point $x' \in   Z'^1_\mathfrak c \cap F'$. Denote with $\mathtt x' : F \to F'$ this map.

Since $\bar \theta$ is a linear preorder, Theorem \ref{T_uniqueness} implies that for all $\mu \in \mathcal P(F)$ and $\nu = (\mathtt x')_\sharp \mu \in \mathcal P(F')$ there exists a unique transference plan $\pi$, given exactly by $(\Id,\mathtt x')_\sharp \mu$. This fact will be used to prove that if $\nu_n \rightharpoonup \mu$ and there exists a $\tilde C^k_0$-finite cost transference plan $\pi_n \in \Pi(\mu,\nu_n)$, then $\pi_n \rightharpoonup \pi$: simply use the l.s.c. of the cost.

The suitable approximating measures are $\nu_n$ locally finitely atomic, and the plans $\pi_n$ minimize the cost
\[
\mathtt c'^k_0(x,x') =
\begin{cases}
|x-x'|^2 & x' - x \in \tilde C'^1_0, \crcr
\infty & \text{otherwise}.
\end{cases}
\]
It can be shown quite easily that the transport problem $\pi_n \in \Pi^{\mathrm{opt}}_{\mathtt c'^k_0}(\mu,\nu_n)$ is solved by a measure concentrated on the graph of a map (because $\mathtt c'^1_0$ is strictly convex), and there are disjoint open regions $\mathcal R_j \subset F$ such that
\[
\pi_n \llcorner_{\mathcal R_j} = (\Id,x_j')_\sharp \mu \llcorner_{\mathcal R_j}.
\]
The point $x_j$ is one of the atoms of $\nu_n$, and moreover the cones $(1-r) \mathcal R_j + r x_j$, $r \in [0,1]$, are disjoint (also by the strict convexity of $\mathtt c'^k_0$). Finally, the set $F \setminus \cup_j \mathcal R_j$ is $\mathcal H^{d-1}$-negligible. We will refer to this structure as a cone vector field.

For a cone vector field, the same estimates on the $\mathcal H^{d-1}$-measure of the set $\cup_j (1-r) \mathcal R_j + r x_j'$ are valid as if there is a single cone, i.e. a set $A$ of positive $\mathcal H^{d-1}$-measure at $0$ has measure
\begin{equation}
\label{E_evol_cone_1}
\mathcal H^{d-1} \big( \cup_j (1-r) \mathcal R_j \cap A + r x_j' \big) = (1-r)^{d-1} \mathcal H^{d-1}(A).
\end{equation}
Due to the convergence of $\pi_n$ to the unique $\pi$, it is a technical argument to show that removing two sets, one negligible for $\mathcal H^{d-1}$ and the other for $\mu$, the estimate \eqref{E_evol_cone_1} pass to the limit with the inequality $\geq$.

At this point it is a standard argument to show that the set of initial and final points have $\mathcal L^d$-measure $0$, and the disintegration of $\mathcal L^d$ on $\tilde Z'^1_\mathfrak c$ is absolutely continuous, of more precisely it is equivalent to $\mathcal H^1$.

Repeating the argument for all dimensions $\ell$ (and taking into account the dependence w.r.t. $\mathfrak a$), we obtain a directed locally affine subpartition $\tilde Z'^\ell_\mathfrak c$, $\tilde C'^\ell_\mathfrak c$ of the fibration $\tilde Z^k_\mathfrak a$, $\tilde C^k_\mathfrak c$.
}

\subsubsection{Conclusion of the argument}
\label{Sss_conclu_argum_fin}


By mapping back the subpartition to the original directed locally affine partition $Z^k_\mathfrak a$, $C^k_\mathfrak a$, we obtain a directed locally affine subpartition $Z'^\ell_\mathfrak c$, $C'^\ell_\mathfrak c$ with the following properties:
\begin{enumerate}
\item the set $\cup Z^k_\mathfrak a \setminus \cup Z'^\ell_\mathfrak c$ is $\delta_1 \times \mathcal H^d$-negligible,
\item the cones $C'^\ell_\mathfrak c$ are extremal subcones of $C^k_\mathfrak a$ (more precisely they are the intersection of $C^k_\mathfrak a$ with the $\ell$-dimensional plane parallel to $Z'^\ell_\mathfrak c$).
\item \label{Point_mini_post}  the set $Z'^\ell_\mathfrak c$ with $\ell = k$ are cyclically connected.
\end{enumerate}
In the case $\bar \mu \ll (\delta_1 \times \mathcal H^d) $, we can repeat the argument until we reach a directed locally affine partition which satisfies Point \eqref{Point_mini_post} above.


\subsection{Structure of the paper}
\label{Ss_structure}


The paper is organized as follows.

In Section \ref{S_setting} we collect some general notations and definitions, in particular the multifunction notation, the definition of the set of linear and affine $k$-dimensional subspaces of $[0,+\infty)\times\R^d$, and some properties of the space $\mathcal C(k,[0,+\infty)\times \R^d)$ of $k$-dimensional non degenerate cones in $[0,+\infty)\times\R^d$. In Section \ref{Ss_partitions_intro} we define the locally affine partitions, and in Section \ref{Ss_measure_transference} we give the basic tools we need of measure theory and optimal mass transportation.

In Section \ref{S_directed_locally_affine_partitions} we give the definition of a directed locally affine partition as a $\sigma$-compact graph $\mathbf D = \{(k,\mathfrak a,Z^k_\mathfrak a,C^k_\mathfrak a)\}$ in the space $\cup_k \big( \{ k \} \times \R^{d+1-k} \times ( [0,+\infty)\times\R^d) \times \mathcal C(k,[0,+\infty)\times\R^d) \big)$, and we show how to divide it into countably many disjoint partitions with the property that each component is closed to a reference plane, a reference cone and contains a given cube. Next, we consider a natural transference cost on the partition, and two measures: a transference plan with cost $\ind_{C_{\mathfrak a}^k}$ and with the first marginal $\bar \mu$ on the set $\mathbf Z_! = (\cup Z^k_\mathfrak a)\cap (\{1\}\times \R^d)$, and the Hausdorff $d-$dimensional measure restricted to $\mathbf Z_1$. We next state the assumptions on the disintegration of $\mathbf H^d \llcorner_{\mathbf Z_1}$, and we show in Section \ref{Ss_mapping_sheaf_to_fibration} that it is equivalent to consider the problem in $\R^{d+1-k} \times \R^k \times \mathcal C(k,\R^k)$, i.e. on a fibration.

In the next Section \ref{S_monotone_relation_on_fibration} we study the transport problem on fibrations, and construct a linear preorder with minimality properties. The construction is based on the notion of set of points $H_w$ which can be reached by axial path from another point $w$. By taking countably many ordered families of $H_{w_n}$ as the parameter of the problem vary, we obtain a family of linear preorders with Borel graph whose equivalence relations generate a $\sigma$-closed family. In Section \ref{Ss_properties_minimal_equivalence_relation} we study the properties of the minimal equivalence relation $\bar E$, which is generated by the pullback of the lexicographic order on the ordinals numbers by a Borel function $\bar \theta$: of particular importance is that the $\mu$-negligible level sets of $\bar \theta$ are uniformly Lipschitz, and that the level set of positive $\mu$-measure are cyclically connected.

With the function $\bar \theta$, in Section \ref{S_decomposition_of_fibration} we show how to construct a directed locally affine subpartition of the original fibration. Section \ref{Ss_definition_transport_initial_etc} we given the definitions of several sets and study their regularity: these sets are needed when defining various subpartitions, Section \ref{Ss_partition_transport_set}. In this construction a residual set $N$ is obtained, and in Section \ref{Ss_analysis_residual_set} we show that it is made of initial and end points, i.e. points which enter the component of the subpartition when following precise directions.
{\color{blue}
In Section \ref{S_disintegration_on_affine} we study the disintegration of the Lebesgue measure on the locally affine subpartition. First we consider the case when the components of the refined partition are directed segments. In Section \ref{Ss_proof_of_cone_property} we prove that in this case the transference plan satisfies a uniqueness property, which implies that the segments can be approximated by piecing together countably many cones, and thus that the estimates on the $\mathcal H^{d-1}$-measure of the sections satisfies some uniform bounds. As a consequence we deduce in Section \ref{Sss_uniform_area_by_cones} that the set of initial and end points is $\mathcal L^d$-negligible, and that the disintegration of the Lebesgue measure satisfies the same regularity assumptions as for the original partition. The extension to the general case (i.e. the components of the partition have dimension $> 1$) is done in Section \ref{Ss_anal_loc_affin_part}.

In the last Section \ref{S_appli_transp_prob} we show has this process can be iterated in order to obtain a partition of $\R^d$ such that each component is cyclically connected. In particular this result can be used for Monge's transportation problem, in order to obtain a decomposition with the same indecomposability property: in particular, for every secondary transference cost, there exists a potential in each of the components of the partition. It is well known that this implies easily the construction of a map.

In Appendix \ref{A_appendix_1} we collect the results on the disintegration of measures, linear preorders and minimality of equivalence relations needed in this paper. Finally, in Appendix \ref{A_appendix_nota} we list the notations used.}
